Faster Algorithms for Quantitative Analysis of Markov Chains and Markov Decision Processes with Small Treewidth

Discrete-time Markov Chains (MCs) and Markov Decision Processes (MDPs) are two standard formalisms in system analysis. Their main associated quantitative objectives are hitting probabilities, discounted sum, and mean payoff. Although there are many techniques for computing these objectives in general MCs/MDPs, they have not been thoroughly studied in terms of parameterized algorithms, particularly when treewidth is used as the parameter. This is in sharp contrast to qualitative objectives for MCs, MDPs and graph games, for which treewidth-based algorithms yield significant complexity improvements. In this work, we show that treewidth can also be used to obtain faster algorithms for the quantitative problems. For an MC with $n$ states and $m$ transitions, we show that each of the classical quantitative objectives can be computed in $O((n+m)\cdot t^2)$ time, given a tree decomposition of the MC that has width $t$. Our results also imply a bound of $O(\kappa\cdot (n+m)\cdot t^2)$ for each objective on MDPs, where $\kappa$ is the number of strategy-iteration refinements required for the given input and objective. Finally, we make an experimental evaluation of our new algorithms on low-treewidth MCs and MDPs obtained from the DaCapo benchmark suite. Our experimental results show that on MCs and MDPs with small treewidth, our algorithms outperform existing well-established methods by one or more orders of magnitude.

==> table-mc-results.tex <==
\begin{tabular}{|r||c|c|c|c|c|c||c|c|c|c|}
	\hline
	\multirow{2}{*}{Benchmark} & \multicolumn{6}{c||}{Hitting Probabilities} & \multicolumn{4}{c|}{Expected Discounted Sum} \\ \cline{2-11} 
	& Ours        & \textsf{Gauss}        & \textsf{Matlab} & \textsf{Gurobi} & \textsf{Prism} & \textsf{Storm}  & Ours & \textsf{Gauss} & \textsf{Matlab} & \textsf{Gurobi}\\ \hline \hline
	xml-apis   &  0.00001  &  0.00001  &  0.20000  &  0.04082  &  0.06000  &  0.01000  &  0.00002  &  0.00001  &  0.09000  &  0.04552\\ \hline 
	xml-apis-1.3.04   &  0.00001  &  0.00001  &  0.13000  &  0.03398  &  0.06200  &  0.02000  &  0.00002  &  0.00001  &  0.11000  &  0.03570\\ \hline 
	dacapo-luindex   &  0.00008  &  0.00020  &  0.06000  &  0.01897  &  0.11800  &  0.01200  &  0.00010  &  0.00020  &  0.09000  &  0.03646\\ \hline 
	dacapo-digest   &  0.00017  &  0.00063  &  0.11000  &  0.08734  &  0.30900  &  0.03000  &  0.00023  &  0.00062  &  0.12000  &  0.05931\\ \hline 
	dacapo-xalan   &  0.00017  &  0.00084  &  0.15000  &  0.11467  &  0.37300  &  0.04000  &  0.00022  &  0.00090  &  0.09000  &  0.05408\\ \hline 
	dacapo-tomcat   &  0.00017  &  0.00062  &  0.17000  &  0.11905  &  0.51400  &  0.05000  &  0.00024  &  0.00059  &  0.13000  &  0.16045\\ \hline 
	dacapo-lusearch   &  0.00030  &  0.00566  &  0.11000  &  0.04260  &  0.57600  &  0.03100  &  0.00039  &  0.00584  &  0.10000  &  0.02560\\ \hline 
	dacapo-lusearch-fix   &  0.00034  &  0.00572  &  0.10000  &  0.03674  &  0.42700  &  0.03200  &  0.00040  &  0.00572  &  0.12000  &  0.04174\\ \hline 
	daytrader   &  0.00020  &  0.00130  &  0.11000  &  0.10136  &  0.66800  &  0.04700  &  0.00028  &  0.00141  &  0.15000  &  0.06834\\ \hline 
	commons-daemon   &  0.00033  &  0.00139  &  0.17000  &  0.21845  &  1.48100  &  0.08400  &  0.00043  &  0.00139  &  0.18000  &  0.18583\\ \hline 
	commons-logging-1.0.4   &  0.00048  &  0.00218  &  0.37000  &  0.42445  &  1.49000  &  0.15000  &  0.00067  &  0.00214  &  0.83000  &  0.35145\\ \hline 
	tomcat-juli   &  0.00058  &  0.00371  &  0.28000  &  0.31819  &  1.61300  &  0.19600  &  0.00078  &  0.00370  &  0.36000  &  0.39547\\ \hline 
	constantine   &  0.00060  &  0.03897  &  0.29000  &  0.25880  &  1.68700  &  0.12900  &  0.00082  &  0.03912  &  0.32000  &  0.27186\\ \hline 
	bootstrap   &  0.00084  &  0.03084  &  0.30000  &  0.22259  &  2.49600  &  0.13000  &  0.00111  &  0.03096  &  0.31000  &  0.22324\\ \hline 
	dacapo-h2   &  0.00104  &  0.01446  &  2.55000  &  0.46082  &  2.22300  &  0.20500  &  0.00160  &  0.01178  &  5.81000  &  0.47357\\ \hline 
	avalon-framework-4.2.0   &  0.00139  &  0.00359  &  1.08000  &  1.16564  &  4.48500  &  0.46400  &  0.00190  &  0.00278  &  1.12000  &  1.24184\\ \hline 
	jnr-posix   &  0.00142  &  0.25385  &  1.23000  &  1.13165  &  7.02200  &  0.78700  &  0.00194  &  0.25623  &  1.42000  &  1.28773\\ \hline 
	commons-logging   &  0.00189  &  0.04127  &  0.84000  &  0.81669  &  4.25500  &  0.38800  &  0.00255  &  0.03683  &  0.42000  &  0.88823\\ \hline 
	jline-0.9.95-SNAPSHOT   &  0.00188  &  0.00793  &  1.41000  &  1.39634  &  8.37200  &  0.91000  &  0.00258  &  0.00788  &  1.65000  &  1.49695\\ \hline 
	asm-commons-3.1   &  0.00217  &  0.03162  &  1.16000  &  1.26295  &  6.18000  &  0.50400  &  0.00288  &  0.03166  &  1.42000  &  1.29334\\ \hline 
	commons-codec   &  0.00257  &  0.03337  &  1.09000  &  0.99834  &  7.50300  &  0.51300  &  0.00398  &  0.03401  &  1.24000  &  0.97073\\ \hline 
	commons-io-1.3.1   &  0.00250  &  0.01205  &  1.36000  &  1.59909  &  8.51900  &  0.68300  &  0.00358  &  0.01210  &  1.22000  &  1.49369\\ \hline 
	asm-3.1   &  0.00285  &  0.13666  &  0.89000  &  0.78284  &  7.46700  &  0.42700  &  0.00380  &  0.13651  &  0.92000  &  0.80580\\ \hline 
	junit-3.8.1   &  0.00322  &  0.00493  &  1.83000  &  3.10246  &  18.74200  &  1.80400  &  0.00423  &  0.00485  &  1.85000  &  3.80143\\ \hline 
	lucene-demos-2.4   &  0.00388  &  0.10829  &  1.09000  &  0.88066  &  7.77000  &  0.67400  &  0.00526  &  0.10898  &  1.07000  &  1.13659\\ \hline 
	jaxen-1.1.1   &  0.00419  &  0.60061  &  2.73000  &  3.44220  &  17.16700  &  1.88600  &  0.00563  &  0.60335  &  2.30000  &  3.22225\\ \hline 
	jaffl   &  0.00522  &  0.09861  &  2.58000  &  3.19677  &  16.49900  &  2.30600  &  0.00706  &  0.09858  &  2.41000  &  3.27322\\ \hline 
	serializer-2.7.0   &  0.00543  &  0.14564  &  1.82000  &  2.36092  &  13.21600  &  1.46200  &  0.00715  &  0.14182  &  2.03000  &  2.86329\\ \hline 
	crimson-1.1.3   &  0.00838  &  0.13650  &  2.48000  &  2.84511  &  17.47500  &  1.43200  &  0.01122  &  0.12941  &  2.25000  &  2.83951\\ \hline 
	commons-httpclient   &  0.00782  &  0.05948  &  4.01000  &  5.60121  &  25.39700  &  2.15900  &  0.01070  &  0.05777  &  3.71000  &  4.89463\\ \hline 
	serializer   &  0.01048  &  0.30260  &  2.63000  &  3.32304  &  32.41300  &  2.59700  &  0.01367  &  0.30280  &  2.60000  &  3.53548\\ \hline 
	janino-2.5.15   &  0.01485  &  0.27481  &  5.38000  &  7.09017  &  57.19600  &  7.69100  &  0.01970  &  0.28066  &  4.35000  &  7.31999\\ \hline 
	xmlgraphics-commons-1.3.1   &  0.01621  &  0.18939  &  5.87000  &  7.08701  &  40.47300  &  5.93600  &  0.02116  &  0.18956  &  6.91000  &  8.74569\\ \hline 
	lucene-core-2.4   &  0.02834  &  1.02118  &  5.16000  &  9.00895  &  71.27600  &  6.56200  &  0.03520  &  0.97595  &  5.90000  &  9.92471\\ \hline 
	xalan-2.6.0   &  0.03358  &  1.77685  &  0.87000  &  15.09464  &  95.42400  &  12.41900  &  0.04760  &  1.77619  &  0.70000  &  17.70531\\ \hline 
	derbyclient   &  0.03198  &  0.59163  &  8.02000  &  16.32040  &  81.51000  &  7.72300  &  0.04193  &  0.59825  &  10.19000  &  16.99502\\ \hline 
	pmd-4.2.5   &  0.03257  &  0.55702  &  9.54000  &  15.22455  &  82.97800  &  10.46600  &  0.04358  &  0.55667  &  10.01000  &  16.07630\\ \hline 
	avrora-cvs-20091224   &  0.03832  &  0.68720  &  3.02000  &  19.21516  &  139.14800  &  8.29700  &  0.05008  &  0.66573  &  2.40000  &  17.86095\\ \hline 
	eclipse   &  0.03693  &  0.50101  &  10.76000  &  16.24855  &  83.30500  &  12.38800  &  0.05109  &  0.49472  &  12.60000  &  14.92674\\ \hline 
	xerces\_2\_5\_0   &  0.05558  &  2.53732  &  12.11000  &  16.05042  &  159.37600  &  22.75000  &  0.07604  &  2.42570  &  13.31000  &  18.45862\\ \hline
\end{tabular}



==> table-mdp-results.tex <==
\begin{tabular}{|r||c|c|c|c|c|c|c|c||c|c|c|c|c|c|}
	\hline
	\multirow{2}{*}{Benchmark} & \multicolumn{8}{c||}{Hitting Probabilities} & \multicolumn{6}{c|}{Expected Discounted Sum} \\ \cline{2-15} 
	& Ours & \textsf{lpsolve} & \textsf{Gurobi} & \textsf{Matlab} & \textsf{SI} & \textsf{VI} & \textsf{Prism} & \textsf{Storm} & Ours & \textsf{lpsolve} & \textsf{Gurobi} & \textsf{Matlab} & \textsf{SI} & \textsf{VI}  \\ \hline \hline
	xml-apis   &  0.00004  &  0.04145  &  0.05033  &  3.06000  &  0.00151  &  0.00072  &  0.07700  &  0.01000  &  0.00015  &  0.03889  &  0.07418  &  2.76000  &  0.00318  &  0.00073\\ \hline 
	xml-apis-1.3.04   &  0.00005  &  0.03836  &  0.04782  &  4.33000  &  0.00157  &  0.00085  &  0.06900  &  0.01200  &  0.00012  &  0.04129  &  0.03201  &  3.11000  &  0.00257  &  0.00076\\ \hline 
	dacapo-luindex   &  0.00033  &  0.02243  &  0.01947  &  5.28000  &  0.00787  &  0.00407  &  0.15300  &  0.00900  &  0.00034  &  0.02059  &  0.02004  &  4.57000  &  0.03685  &  0.00431\\ \hline 
	dacapo-digest   &  0.00101  &  0.05517  &  0.09404  &  8.66000  &  0.01816  &  0.00800  &  0.28000  &  0.02600  &  0.00149  &  0.05713  &  0.07190  &  6.46000  &  0.03654  &  0.00978\\ \hline 
	dacapo-xalan   &  0.00069  &  0.07645  &  0.11382  &  7.83000  &  0.01703  &  0.01001  &  0.33700  &  0.02600  &  0.00507  &  0.07229  &  0.10148  &  5.94000  &  0.01549  &  0.01208\\ \hline 
	dacapo-tomcat   &  0.00180  &  0.12966  &  0.18451  &  9.20000  &  0.01916  &  0.00863  &  0.50000  &  0.04600  &  0.00151  &  0.13067  &  0.18988  &  7.84000  &  0.16863  &  0.01018\\ \hline 
	dacapo-lusearch   &  0.00160  &  0.03950  &  0.04988  &  10.55000  &  0.03473  &  0.01553  &  0.34700  &  0.02400  &  0.00239  &  0.03813  &  0.03714  &  8.60000  &  0.04062  &  0.01653\\ \hline 
	dacapo-lusearch-fix   &  0.00516  &  0.04036  &  0.05746  &  8.58000  &  0.02918  &  0.01441  &  0.33600  &  0.02700  &  0.00248  &  0.03770  &  0.04122  &  7.94000  &  0.04010  &  0.02004\\ \hline 
	daytrader   &  0.00073  &  0.08304  &  0.09799  &  8.95000  &  0.03308  &  0.01531  &  0.48600  &  0.03900  &  0.00134  &  0.09054  &  0.08769  &  8.17000  &  0.04721  &  0.01626\\ \hline 
	commons-daemon   &  0.00271  &  0.22508  &  0.23568  &  9.18000  &  0.03780  &  0.01816  &  1.26900  &  0.08000  &  0.00335  &  0.19132  &  0.29852  &  11.59000  &  0.08002  &  0.01998\\ \hline 
	commons-logging-1.0.4   &  0.00175  &  0.38711  &  0.54011  &  19.48000  &  0.12354  &  0.04529  &  1.96100  &  0.13300  &  0.00382  &  0.33759  &  0.53407  &  12.68000  &  0.15830  &  0.03233\\ \hline 
	tomcat-juli   &  0.00325  &  0.27254  &  0.44136  &  12.79000  &  0.06386  &  0.03181  &  1.37400  &  0.15300  &  0.00558  &  0.37249  &  0.48284  &  11.54000  &  0.15890  &  0.20590\\ \hline 
	constantine   &  0.00349  &  0.24723  &  0.33957  &  17.65000  &  0.09099  &  0.03940  &  1.30000  &  0.10000  &  0.00678  &  0.23486  &  0.28992  &  12.54000  &  0.35064  &  0.05305\\ \hline 
	bootstrap   &  0.00788  &  0.23418  &  0.28990  &  17.02000  &  0.12021  &  0.05957  &  1.41200  &  0.10100  &  0.00762  &  0.20695  &  0.26406  &  15.08000  &  0.15577  &  0.07828\\ \hline 
	dacapo-h2   &  0.00507  &  0.44370  &  0.52646  &  22.39000  &  0.13434  &  0.06553  &  1.91600  &  0.16200  &  0.00838  &  0.42674  &  0.54066  &  20.75000  &  0.16036  &  0.07301\\ \hline 
	avalon-framework-4.2.0   &  0.00505  &  1.08039  &  1.35913  &  27.85000  &  0.15185  &  0.07622  &  4.86800  &  0.45100  &  0.01810  &  1.20308  &  1.50038  &  22.67000  &  0.31613  &  0.08697\\ \hline 
	jnr-posix   &  0.01413  &  1.20555  &  1.52360  &  23.05000  &  0.22817  &  0.11717  &  5.74900  &  0.45500  &  0.01688  &  1.23360  &  1.81516  &  21.60000  &  0.37101  &  0.12226\\ \hline 
	commons-logging   &  0.00904  &  0.80701  &  1.00470  &  29.37000  &  0.25868  &  0.11347  &  3.92900  &  0.31700  &  0.02875  &  0.72560  &  0.98885  &  25.38000  &  1.38934  &  0.13886\\ \hline 
	jline-0.9.95-SNAPSHOT   &  0.01112  &  1.48252  &  2.02085  &  20.62000  &  0.20213  &  0.10417  &  6.44600  &  0.55000  &  0.02444  &  1.68731  &  2.18862  &  32.36000  &  0.46697  &  0.14053\\ \hline 
	asm-commons-3.1   &  0.01002  &  1.20580  &  1.55601  &  21.84000  &  0.22011  &  0.10860  &  7.09800  &  0.45600  &  0.01669  &  1.32881  &  2.02500  &  37.33000  &  0.64163  &  0.13915\\ \hline 
	commons-codec   &  0.01272  &  1.18706  &  1.37049  &  20.03000  &  0.31467  &  0.15661  &  6.59400  &  0.49500  &  0.02478  &  1.01284  &  1.32599  &  37.47000  &  0.62215  &  0.15808\\ \hline 
	commons-io-1.3.1   &  0.01134  &  1.70944  &  2.15621  &  48.41000  &  0.29763  &  0.13720  &  6.84900  &  0.57600  &  0.02544  &  1.49117  &  2.22190  &  25.90000  &  1.05737  &  0.15389\\ \hline 
	asm-3.1   &  0.01298  &  0.75230  &  0.98912  &  17.84000  &  0.38381  &  0.20731  &  7.38900  &  0.36200  &  0.02566  &  0.80930  &  1.20244  &  39.74000  &  1.53952  &  0.66412\\ \hline 
	junit-3.8.1   &  0.01116  &  3.28112  &  4.48130  &  48.02000  &  0.28184  &  0.17565  &  12.72300  &  1.24400  &  0.02967  &  3.43031  &  4.54870  &  54.49000  &  1.61903  &  0.19736\\ \hline 
	lucene-demos-2.4   &  0.01978  &  0.92039  &  1.17712  &  40.06000  &  0.67695  &  0.26995  &  6.27900  &  0.54500  &  0.04212  &  0.98169  &  1.38443  &  41.28000  &  1.68492  &  0.55803\\ \hline 
	jaxen-1.1.1   &  0.02025  &  3.17878  &  4.08971  &  41.38000  &  0.62182  &  0.27318  &  15.28600  &  1.17500  &  0.05828  &  3.11529  &  4.00512  &  55.82000  &  7.40472  &  0.34462\\ \hline 
	jaffl   &  0.03770  &  3.05149  &  4.26184  &  59.08000  &  0.65796  &  0.31335  &  16.27800  &  1.42100  &  0.04769  &  3.31774  &  4.50510  &  60.56000  &  1.83675  &  4.18679\\ \hline 
	serializer-2.7.0   &  0.02506  &  2.09810  &  3.66582  &  52.06000  &  0.60972  &  0.31064  &  11.33300  &  1.05700  &  0.04071  &  2.67593  &  3.72690  &  38.10000  &  1.52886  &  0.43002\\ \hline 
	crimson-1.1.3   &  0.05404  &  2.58277  &  3.86147  &  92.63000  &  1.76648  &  0.64496  &  15.51500  &  1.21000  &  0.10414  &  2.85201  &  3.47488  &  72.86000  &  3.67908  &  0.50956\\ \hline 
	commons-httpclient   &  0.03319  &  5.54198  &  6.69283  &  117.38000  &  1.05233  &  0.46138  &  22.27200  &  1.81400  &  0.06327  &  4.79292  &  6.92428  &  78.85000  &  2.95078  &  0.55254\\ \hline 
	serializer   &  0.07065  &  2.91949  &  4.32873  &  56.01000  &  1.28958  &  0.64523  &  25.73500  &  2.00500  &  0.10003  &  3.85245  &  5.27190  &  64.05000  &  2.57026  &  0.88358\\ \hline 
	janino-2.5.15   &  0.07314  &  6.68790  &  9.91680  &  145.83000  &  2.01809  &  1.13186  &  34.01700  &  3.00600  &  0.13146  &  6.94878  &  9.30685  &  133.24000  &  5.84305  &  1.23715\\ \hline 
	xmlgraphics-commons-1.3.1   &  0.07193  &  8.19395  &  11.86806  &  79.65000  &  1.90528  &  0.92933  &  39.59300  &  4.93900  &  0.15004  &  8.27969  &  11.30344  &  144.15000  &  15.20058  &  1.08951\\ \hline 
	lucene-core-2.4   &  0.16863  &  9.23440  &  12.98207  &  322.52000  &  2.92001  &  1.61256  &  52.34900  &  4.53700  &  0.29733  &  8.68221  &  12.39745  &  189.91000  &  7.40384  &  2.24896\\ \hline 
	xalan-2.6.0   &  0.15804  &  13.00583  &  23.80962  &  275.80000  &  4.77874  &  2.50689  &  77.43000  &  9.28700  &  0.30192  &  16.62097  &  21.80253  &  208.95000  &  15.14658  &  2.59791\\ \hline 
	derbyclient   &  0.12489  &  16.30398  &  20.86866  &  256.40000  &  3.77297  &  1.76492  &  87.46500  &  6.32500  &  0.25004  &  15.75678  &  19.19841  &  303.18000  &  14.63486  &  2.18177\\ \hline 
	pmd-4.2.5   &  0.14238  &  13.77016  &  21.09903  &  512.47000  &  5.27168  &  2.25309  &  84.40400  &  7.07000  &  0.25993  &  17.26150  &  21.83183  &  240.07000  &  17.99462  &  2.84897\\ \hline 
	avrora-cvs-20091224   &  0.13498  &  18.70873  &  24.66722  &  290.39000  &  4.39129  &  2.03788  &  101.28400  &  7.92000  &  0.25995  &  19.79896  &  25.89820  &  389.31000  &  19.05126  &  2.56352\\ \hline 
	eclipse   &  0.25944  &  14.32922  &  20.26574  &  406.15000  &  6.40507  &  2.76358  &  104.00300  &  6.65400  &  0.55813  &  14.74519  &  17.84516  &  598.65000  &  15.26801  &  3.71952\\ \hline 
	xerces\_2\_5\_0   &  0.34422  &  14.79255  &  22.62586  &  257.56000  &  9.89841  &  4.58320  &  126.73300  &  12.73800  &  0.46794  &  17.21913  &  24.70113  &  320.46000  &  38.72352  &  4.46858 \\ \hline
\end{tabular}
